Automated Synthesis of Safe and Robust PID Controllers for Stochastic Hybrid Systems

We present a new method for the automated synthesis of safe and robust Proportional-Integral-Derivative (PID) controllers for stochastic hybrid systems. Despite their widespread use in industry, no automated method currently exists for deriving a PID controller (or any other type of controller, for that matter) with safety and performance guarantees for such a general class of systems. In particular, we consider hybrid systems with nonlinear dynamics (Lipschitz-continuous ordinary differential equations) and random parameters, and we synthesize PID controllers such that the resulting closed-loop systems satisfy safety and performance constraints given as probabilistic bounded reachability properties. Our technique leverages SMT solvers over the reals and nonlinear differential equations to provide formal guarantees that the synthesized controllers satisfy such properties. These controllers are also robust by design since they minimize the probability of reaching an unsafe state in the presence of random disturbances. We apply our approach to the problem of insulin regulation for type 1 diabetes, synthesizing controllers with robust responses to large random meal disturbances, thereby enabling them to maintain blood glucose levels within healthy, safe ranges.

==> ap_intro.tex <==
We evaluate our method on the closed-loop control of insulin treatment for Type 1 diabetes (T1D), also known as the \textit{artificial pancreas (AP)}~\cite{hovorka2011closed}. Together with model predictive control, PID is the main control technique for the AP~\cite{steil2011effect,huyett2015design}, and is found as well in commercial devices~\cite{kanderian2014apparatus}. 
%For their potential to improve the life of diabetic patients by overcoming manual insulin dosing, AP systems have been extensively studied in the past 20 years~\cite{hovorka2011closed}, but only lately cleared for clinical trials~\cite{ly2015day,kovatchev2017feasibility} and commercialization \cite{kanderian2010apparatus,kanderian2014apparatus}. 

The main requirement for the AP is to keep blood glucose (BG) levels within tight, healthy ranges, typically between 70-180 mg/dL, in order to avoid \textit{hyperglycemia} (BG above the healthy range) and \textit{hypoglycemia} (BG below the healthy range). While some temporary, postprandial hyperglycemia is typically admissible, hypoglycemia leads to severe health consequences, and thus, it should be avoided as much as possible. This is a crucial safety requirement, which we will incorporate in our synthesis properties.

The AP consists of a continuous glucose monitor that provides glucose measurements to a control algorithm regulating the amount of insulin injected by the insulin pump. 
%running inside an insulin pump, which is a wearable device that injects insulin inside the body. 
The pump administers both \textit{basal insulin}, a low and continuous dose that covers insulin needs outside meals, and \textit{bolus insulin}, a single high dose for covering meals. 

Meals represent indeed the major disturbance in insulin control, which is why state-of-the-art commercial systems\footnote{MINIMED 670G by Medtronic \url{https://www.medtronicdiabetes.com/products/minimed-670g-insulin-pump-system}} can only regulate basal insulin and still require explicit meal announcements by the patient for bolus insulin. To this purpose, robust control methods have been investigated \cite{parker2000robust,szalay2014linear,paolettiCMSB17}, since they are able to minimize the impact of input disturbances (in our case, meals) on the plant (the patient). Thus, they have the potential to provide full closed-loop control of bolus insulin without manual dosing by the patient, which is inherently error-prone and hence dangerous. Our method for the synthesis of safe and robust controllers is therefore particularly meaningful in this case. 


==> macros.tex <==
% GENERIC MATH MACROS
%\newcommand{\eventually}{\Diamond}
\newcommand{\henceforth}{\Box}
\newcommand{\tuple}[1]{\langle #1\rangle}
\newcommand{\sat}{\models}
% \pr(X) = probability of X.  it's probably a good idea to use same font
% for \pr and \Peek.
\newcommand{\pr}{{\it P}}
\newcommand{\Peek}{{\it Peek}}
\newcommand{\comment}[1]{}

% \fullOnly{material that appears in tech report but not conference paper}
\newcommand{\fullOnly}[1]{}
%\newcommand{\fullOnly}[1]{#1}

% \confOnly{material that appears in conference paper but not tech report}
%\newcommand{\confOnly}[1]{}
\newcommand{\confOnly}[1]{#1}

% DOCUMENT-SPECIFIC MACROS
% observation symbol representing a gap
\newcommand{\gap}{{\it gap}}
% random variable representing the result of a peek operation.
% use regular font not \mathbf, i.e., assume a single variable,
% otherwise it looks odd, because X, O, and S are single variables.
\newcommand{\pkvar}{Q}
% meta-variable representing a value returned by a peek operation,
% i.e., a value of \pkvar.
\newcommand{\pk}{q}

% \sampled{O} = sampled version of trace O
%\newcommand{\samp}[1]{\check{#1}}
%\newcommand{\samp}[1]{{\rm samp}(#1)}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> steady_state.tex <==
%\subsubsection{Basal insulin rate synthesis and steady state approximation}
\subsubsection{Basal insulin rate synthesis and steady state computation}
%The basal insulin rate $u_b$ is a constant rate at which insulin is administered
%and for which the system (\ref{eq:model-odes}) reaches 
%the steady state determined by the equation $Q_1(t) = sp$.
Formally, the basal insulin rate $u_b$ is the constant infusion rate that, without meal disturbances ($D_G=0$), 
keeps the gluco-regulatory system to the steady state determined by $Q_1(t) = sp$. 

%a constant rate at which insulin is administered
%and for which the system (\ref{eq:model-odes}) reaches 
%the steady state determined by the equation $Q_1(t) = sp$.

The aim of this experiment is two-fold: 1) synthesis of the basal rate value $u_b$ for which
the system of ODEs (\ref{eq:model-odes}) reaches the steady state and 
2) %obtaining the approximate value of the steady state of the system (\ref{eq:model-odes}).
computing this steady state. 


Starting with $Q_1(0) = sp$ and 0 for the remaining 
differential equations, 
we applied the formal approach of ProbReach to synthesize a value for $u_b$ 
such that the output glucose $Q_1$ 
%we obtained the range of values for $u_b$
%for which the value of $Q_1$ 
reaches the interval $[sp-0.5,sp+0.5]$
in 2,000 minutes and remains there for the following 1,000 minutes. 
Since any reasonable basal rate cannot exceed 1 unit of insulin per minute, we considered the domain $[0,1]$ for $u_b$, 
from which the synthesis algorithm returned the feasible interval $[0.0553359375, 0.055640625]$. 
%The basal insulin rate synthesis was performed by applying the formal approach of ProbReach  
%to the interval $[0,1]$, and the interval $[0.0553359375, 0.055640625]$ 
%was identified as feasible.
Due to the absolute guarantees provided by the formal technique,
the property above is satisfied for any value in the obtained interval.
We will use $u_b=0.0555$ for all further experiments. 

Then, given the basal infusion rate $u_b=0.0555$, we obtained the %approximate 
value of the system's steady state as the value of the system's dynamics at 
$t=3,000$ minutes (see Table \ref{table:steady}). 
We use the system's steady state as the initial state in all further experiments. 

We denote with $C_0$ the basal controller that switches off the PID controller and applies only $u_b$. 

\begin{table}[ht!]
\centering
\begin{tabular}{|c|c||c|c||c|c|}
\hline
\bf{var} & \bf{value} & \bf{var} & \bf{value} & \bf{var} & \bf{value} \\
\hline
\hline
$Q_1$ & $sp$ & $Q_2$ & 19.08024 & $S_1$ & 3.0525 \\ 
$S_2$ & 3.0525 & $I$ & 0.03351 & $x_1$ & 0.01899 \\ 
$x_2$ & 0.03128 & $x_3$ & 0.02681 & & \\ 
\hline
\end{tabular}
\vspace{2ex}
\caption{Approximate value of the steady state of the ODE system (\ref{eq:model-odes})
for the given set point $sp$.}
\label{table:steady}
\end{table}
